Explainable AI Enabled Inspection of Business Process Prediction Models

Modern data analytics underpinned by machine learning techniques has become a key enabler to the automation of data-led decision making. As an important branch of state-of-the-art data analytics, business process predictions are also faced with a challenge in regard to the lack of explanation to the reasoning and decision by the underlying `black-box' prediction models. With the development of interpretable machine learning techniques, explanations can be generated for a black-box model, making it possible for (human) users to access the reasoning behind machine learned predictions. In this paper, we aim to present an approach that allows us to use model explanations to investigate certain reasoning applied by machine learned predictions and detect potential issues with the underlying methods thus enhancing trust in business process prediction models. A novel contribution of our approach is the proposal of model inspection that leverages both the explanations generated by interpretable machine learning mechanisms and the contextual or domain knowledge extracted from event logs that record historical process execution. Findings drawn from this work are expected to serve as a key input to developing model reliability metrics and evaluation in the context of business process predictions.

==> sections/sketch.tex <==
We further analyse \textit{prefix\_agg} method where a classifier XGBoost is trained for each bucket containing traces of certain, pre-defined prefix lengths. Global and local explanations for buckets containing prefixes of length $5$ and $10$ are shown in Fig.~\ref{fig:bpic2012_prefix_agg}. %Buckets with lower prefix lengths use information of the trace executed thus far. 
Global explanations indicate that the important features are resources executing the activities (Fig.~\ref{fig:bpic2012_prefix_agg}(a) and (c)). 
Local explanations provide some interesting insights: lower values of the features (such as \textit{the time since last event}, \textit{the time since the case started}) increase the likelihood of the positive outcome (Fig.~\ref{fig:bpic2012_prefix_agg}(b) and (d)). While a \textit{prefix\_agg} method has generally lower accuracy (refer to AUC plots in Fig.~\ref{fig:bpic2012_agg_single_prefix}(a)), it uses features that can be computed based on the activities executed in the running case of a given prefix length and hence would be better suited for traces with lower prefix lengths. 
%Lipton~\cite{lipton2018} e.g. the standard deviation of activity duration, minimum number of open cases when the event is executing. 

\begin{figure}[t!]
		\vspace*{.5\baselineskip}
		\resizebox{\textwidth}{!}{\centering\includegraphics{figures/bpic2012_prefix_agg}}
		\caption{Interpreting outcome prediction using \textit{bpic2012\_1} event log: (a)-(d) global and local explanations for \textit{prefix\_agg} method with prefix lengths $5$ and $10$.} 
\label{fig:bpic2012_prefix_agg}
\end{figure}


% ---------- Analysis~3 ---------- \\
\subsubsection{Analysing relevance of multi-perspective features?}

The purpose of this analysis is to reason the relevance of the features identified important for process prediction. Feature importance in global explanations and feature impact to predictions of traces in local explanations are valuable inputs to interpreting feature relevance. To derive such interpretation a good understanding of the business process is often needed. Below, we discuss two examples of applying \textit{single\_agg} with XGBoost to remaining time prediction using \textit{bpic2011} and \textit{bpic2012o} event logs, respectively. 

For \textit{bpic2011} log, it can be observed that, from the local explanation shown in Fig.~\ref{fig:bpic2011_tp}(c), the predictive model relies on features such as \texttt{Diagnosis Treatment Combination ID}, \texttt{Treatment code} and \texttt{Diagnosis code} in order to determine the remaining time of the case. For a regression problem, like time prediction, this explanation indicates that the model is relying mostly on \textit{static} features, which are the features that do not change throughout the lifetime of a case. The usage of static features for regression suggests that the process execution does not rely on the executions of activities or cases (i.e., sequences of activities following different control-flow logics) and that the model uses attributes that do not change during the case execution when making a prediction. % (data perspective). 
Another interesting observation is from the global explanation shown in Fig.~\ref{fig:bpic2011_tp}(b), which indicates that the most significant feature for remaining time prediction is \texttt{Diagnosis\_code = DC822}. By applying statistical analysis on the event log, as depicted in Fig.~\ref{fig:bpic2011_tp}(d), we discovered that 82\% of the events associated with this diagnosis code had the feature \texttt{elapsed time = 0}, which means that the corresponding activity starts and ends immediately. To this end, lack of relevant knowledge about the business process limits our ability to derive further insights about the relationship between these static diagnosis codes, with 0-valued elapsed times and its relation with the remaining time of a running case of the process.

% ------ It also raises an important question as to when the case attributes are available during the execution of a case. If all the case attributes are not available during the beginning of a case execution but are available as the case executes, prefix length bucket would be more appropriate to use rather than a single bucket. Hence, such interpretations are useful in choosing the right bucketing techniques. ------ moved to Discussions section

For \textit{bpic2012o} log, the analysis leads to different observations. As shown in Fig.~\ref{fig:bpic2012O_tp}, the global explanation and the local explanation for trace of prefix length $12$ indicate the resource perspective of the business process are the important features used by the predictive model and have a positive impact on the remaining time prediction. The features identified as highly relevant may be case-related (such as \texttt{agg\_opencases}), resource-related (such as \texttt{agg\_resource}), or time-dependent (such as \texttt{agg\_elapsed time}). It is worth noting that the features like \texttt{agg\_opencases} and \texttt{agg\_elapsed time}, which have a positive impact on the performance of the predictive model, are not among the data attributes of the original event log and are introduced during feature encoding. These features are known as engineered features. One potential problem with introducing engineered features is that they might contribute to the loss of interpretability of a regression model~\cite{lipton2018}. However, the features that are engineered in a meaningful way may be aligned with understanding of the business process, in which case, it is likely that they may be interpretable given relevant process knowledge. %The features further enable the extraction of meaningful insights from the regression model that enable us to assess the trustworthiness of the model.

\begin{figure}[h!]
		\vspace*{-.5\baselineskip}
    \resizebox{\textwidth}{!}{\includegraphics{figures/bpic2012o_single_agg}}
    \caption{Interpreting remaining time prediction for \textit{bpic2012o} event log using \textit{single\_agg} with XGBoost: (a) global explanation and (b) local explanation for prefix length $12$.}
\label{fig:bpic2012O_tp}
\end{figure}



\subsection{Other scenarios: may not include} 

\subsubsection{Analysis~2: Aggregation encoding vs. index encoding.} 

This is to compare the two different feature encoding techniques in terms of their impact on predictions. Based on the findings in Analysis~1, we use prefix-length bucket and apply the following two combinations with XGBoost models to \textit{bpic2012\_1} event log for outcome prediction: i) prefix bucket and aggregation encoding (\textit{prefix\_agg}) and ii) prefix bucket and index encoding (\textit{prefix\_index}). Both models are of similar accuracy according to the AUC plots shown in Fig.~\ref{fig:bpic2012_agg_single_prefix}(a). 

Fig.~\ref{fig:bpic2012_prefix_index}(a) and~(c) illustrate the global explanations of the model trained at distinct prefix lengths ($5$ and $10$) using index encoding, which show that the model used activity or resource information about the prior events. The features used by the model are similar to the aggregation encoding for prefix-length buckets (refer to Fig.~\ref{fig:bpic2012_prefix_agg}(a) and~(c)). The models trained on lower prefix lengths (e.g., $5$) use information about the resources executing activities at certain indexes (temporally ordered). 

While both \textit{prefix\_agg} and \textit{prefix\_index} use information of the resources, the resource values used by the models are different. In this scenario, we are unable to conclude which model provides better explanations limited by our knowledge of the business process. However, since the index encoding uses attributes at each index, the number of features can be very high for processes that have large number of activities, resources and data attributes. The accuracy of the model could deteriorate in those situations as observed in the benchmark results presented in~\cite{teinemaa2019}. Hence, aggregation encoding would be considered more suitable when dealing with business processes with large number of activities, resources and data attributes.

\begin{figure}[t!]
		\vspace*{.5\baselineskip}
		\resizebox{\textwidth}{!}{\centering\includegraphics{figures/bpic2012_prefix_index}}
		\caption{Interpreting outcome prediction using \textit{bpic2012\_1} event log: (a)-(d) global and local explanations for \textit{prefix\_index} method with prefix lengths $5$ and $10$.}
\label{fig:bpic2012_prefix_index}
\end{figure}

\subsubsection{Analysis~3: One-hot data encoding.} 

In both process outcome and remaining time predictions, the aggregation and index encoding techniques further apply one-hot data encoding (or, one-hot encoding) to represent the activities, resources and other categorical data from the event log to feature vectors as input for machine learning models. The purpose of this analysis is to understand the impact of one-hot encoding on the predictive methods being studied. 

In principle, one-hot encoding increases the size of a dataset exponentially, because each attribute value of a feature becomes a new feature by itself with the possible value of $0$ or $1$. For instance, a feature~$F$ with three attributes values $f_1$, $f_2$ and $f_3$ will be represented as three new binary features. This data encoding method generates very sparse datasets, which impacts negatively both the performance metrics of the prediction model and the ability to generate interpretations. Below we discuss the findings that were obtained from analysing the explanations derived from applying \textit{single\_agg} with XGBoost model to process remaining time prediction using \textit{bpic2011} event log as an example. %and \textit{bpic2012o} event logs . %and \textit{bpic2015\_5}.

Fig.~\ref{fig:bpic2011_tp} depicts certain impact of one-hot encoding in the context of \textit{bpic2011} log. The original dataset increased from approximately 20 features to 823 features with this representation (see a snapshot of feature matrix in Fig.~\ref{fig:bpic2011_tp}(a)). Further, a majority of the local explanations can be represented as the follows: \textit{if feature~$X$ is absent (value $\leq 0$), then it influences the remaining time prediction}. When a dataset is so sparse, it is reasonable to expect such type of explanations. However, the question that may arise from this finding is: \textit{To what extent can this provide a meaningful understanding of why the predictive model made a certain prediction?}

%This analysis is further extended to the \textit{bpic2012o} event log (Fig.~\ref{fig:bpic2012O_tp}). In this event log, the predictive model learned to ignore the sparse features and used time-dependent features or dynamical features. It raises an important question on the need to add sparse vectors and raise the complexity of the model input, when the core of the regression model is in a limited number of time-dependent features. In summary, one-hot encoding is a technique that should be used only for very large datasets. For event logs with small size, this technique is not advantageous to represent the data.

\begin{figure}[b!]
%		\vspace*{.5\baselineskip}
    \resizebox{\textwidth}{!}{\centering\includegraphics{figures/bpic2011_single_agg}}
    \caption{Interpreting remaining time prediction for \textit{bpic2011} event log using \textit{single\_agg} with XGBoost: (a) data sparsity as result of one-hot encoding; (b) global explanation; (c) local explanation for trace of prefix length of $12$; and (d) normalised elapse time for a specific diagnosis code.}
\label{fig:bpic2011_tp}
\end{figure}


%Model explanations further provide an understanding of the different perspectives of the business process knowledge used in the outcome prediction. 
%The BPIC 2011 log has the outcome label set as positive based on the occurrence of an event (specific activity) in a trace. We use the prefix length bucket and aggregation encoding to identify features responsible for predicting the outcome. Prefix lengths of 10 and 25 are used to depict two scenarios as the case progresses. As seen in Fig.~\ref{fig:bpic2011_prefix_static1}, the model predominantly uses the static attributes or the attribute of the first event that remain the same throughout the execution of the trace. Use of case attributes indicates limited use of activity information or the control-flow perspective.  The local explanations provide similar insight on the the use of static case attributes for making a prediction. The process model reveals that the activity is one of the first possible events after the start event and hence the model is not influenced activity occurrences.

%\begin{figure}[!h]
%  \resizebox{\textwidth}{!}{\centering\includegraphics{figures/bpic2011_static_features.jpg}}
%    \caption{Global and local explanations for prefix lengths 10 and 25 on BPIC 2011 log.}
%    \label{fig:bpic2011_prefix_static1}
%\end{figure}
%\vspace*{-1\baselineskip}



%To understand the predictions for a single trace, we use LIME~\cite{Ribeiro16} and generate \textit{local explanations} for a few randomly chosen traces that have a positive outcome label (outcome=1). Fig.~\ref{fig:bpic2015_agg_single} further presents explanations for three traces with a positive label having the prefix length of 5, 10, and 25, respectively.  The green bar in the figure shows the feature and the expression it satisfies that increases the prediction probability of the positive class label, while the red bars indicate the feature and the expression it satisfies that reduces prediction probability of the positive class label. The local explanations for prefix length 5 and 10 show why the model predicted the outcome incorrectly. From the explanations it can be seen that the model relies on the two activities. Their non-occurrence (\texttt{08\_AWB45\_010 <=0}) leads to an incorrect prediction by the model for the prefix length of 5 and 10. The occurrence of the activity for prefix length 25 results in a correct outcome prediction. The local explanations reveal that the model is influenced by the occurrence of two activities or features (highly) correlated to the output, once again confirming the data leakage.

%\paragraph{\bf Interpreting features used for remaining time prediction:}
%
%To verify if performance metrics such as \textit{MAE} is sufficient, we analyze the best performing predictive model with low \textit{MAE} on the event logs \textit{bpic2011} and \textit{bpic2012o}. Figures~\ref{fig:bpic2011_tp} and~\ref{fig:bpic2012O_tp} show this analysis, respectively.
%
%In Fig.~\ref{fig:bpic2011_tp}, one can see that the algorithm relies on features such as \textit{Diagnosis Treatment Combination ID}, \textit{Treatment code} and \textit{Diagnosis} in order to determine the remaining time of the case. For a regression task, like time prediction, this explanation indicates that the model is relying mostly on static features; in other words, features that do not change much throughout the lifetime of a case. The usage of static features for regression thus suggests that the process execution does not rely on the case activities or case execution (control-flow) and that the model uses attributes that do not change during the case execution when making a prediction (data perspective). It also raises an important question as to when the case attributes are available during the execution of the case. If all the case attributes are not available during the beginning of a case execution but are available as the case executes, prefix length bucket would be more appropriate to use rather than a single bucket. Hence, such interpretations are useful in choosing the right bucketing techniques.
%
%The analysis of \textit{bpic2012o} leads to different observations. In this event log, the explanations indicate the resource perspective of the process model are the important features used by the predictive model and have a positive impact on the prediction of the remaining time of the process. Some of the features identified as highly relevant are either dynamic, like \texttt{agg\_opencases} and \texttt{agg\_resource}, or time-dependent, such as \texttt{agg\_elapsed time}. Although the features \texttt{agg\_opencases} and \texttt{agg\_elapsed time} are not part of the original event log and are additionally introduced, these features have a positive impact on the performance of the classifier. One potential problem with adding engineered features is that they might contribute to the loss of interpretability of the regression model~\cite{lipton2018}. However, the features are engineered in a meaningful way and are aligned with understanding the business process. The features further enable the extraction of meaningful insights from the regression model that enable us to assess the trustworthiness of the model.

%\paragraph{\bf Interpreting encoding techniques:}
%
%\paragraph{\bf Interpreting business process knowledge used by a predictive model:}
%
%An understanding of the business process is vital when it comes to the generation of predictive models because it enables the assessment of whether a performance metric makes a good representation of the underlying business process or not. For example, in the bpic2011 event log, a set of engineered features, such as max/mean/std. deviation of elapsed time, were added to enrich the event log. Paradoxically, the regression models did not use a single time-dependent feature in the prediction of the remaining time of the process. Fig.~\ref{fig:bpic2011_tp}, indicates that the most significant feature for remaining time prediction is the \texttt{Diagnosis Code = DC822}. In our analysis, we discovered that 82\% of the events associated with the diagnosis code had the feature \texttt{elapsed time = 0}, which means that the activity starts and ends immediately. Lack of business process knowledge limits the ability to provides us deep insights about the relationship between these static diagnosis codes, with 0-valued elapsed times and its relation with the remaining time of the process.
%
%It is acknowledged in the literature that human decisions are also opaque (or a black box)~\cite{Holzinger19}, meaning that, under uncertainty, humans make their decisions not only based on data, but also based on intuitions, emotions, feelings, etc. This implies that human decision-making is highly susceptible to cognitive bias and these biases will be manifested in human recorded data. Machine learning algorithms that operate over such data will lead to biased results, which are hard for the decision-maker to identify due to the black-box nature of these algorithms. 



%in the context of two existing process monitoring benchmarks.  

%we derive global and local explanations of selected prediction models using interpretable machine learning techniques, extract process knowledge using process mining techniques, and then conduct analyses of the derived interpretations to draw interesting findings about these predictive models. 

%In this section, we aim to interpret and gain deeper insights into the predictive models 

%the following three aspects: first, we derive explanations and analyse the influence of different bucketing and encoding methods on model predictions, thus evaluating the suitability of different feature representation mechanisms; second, we investigate the influence of event attributes on the model prediction. 

%This section presents a summary of our findings on investigating the suitability of various feature encoding and bucketing techniques used for predicting process outcome. Multiple encoding and bucketing methods representing the event log have been prescribed and evaluated for accuracy in previous studies~\cite{teinemaa2019}. 
%We aim to derive global and local interpretations for the predictive models and gain deeper insights of the features used by the model for making a prediction. These explanation s can be used to assess the suitability of the bucketing or encoding methods when predicting outcomes of a specific process. 

%This section presents the results of the explanations for the task of remaining time prediction. The task of remaining time prediction can be defined in the following way: ``Given an event log of complete cases of a business process, and a prefix case of this process as obtained from an event stream, we want to predict a performance measure of such prefix case in the future''~\cite{verenich2019}. An example of such a performance measure is the prediction of the time that remains for a case to be completed. %The explanations are generated for the three logs in Section 3: the \textit{BPIC2011}, \textit{BPIC2012} and \textit{BPIC2015}. 
%The regression model XGBoost is used with the bucketing and encoding methods detailed in Section~\ref{subsec:approach}. Due to space limitations, we present the key insights drawn from the model explanations. 

% Though these findings are not yet generalised, they motivate the need to derive explanations which are useful in identifying a suitable predictive model while not limiting the choice based on only the accuracy. 

%An overall workflow of predictive analytics used in the context of process monitoring is illustrated in Fig.~\ref{fig:prediction_workflow}. 

%More specifically, a \textit{trace}~$\sigma$ is a sequence of \textit{events} of the same case. During the training phase, \textit{prefixes} are generated for each trace. A prefix function $\mathit{prefix}(\sigma,l)$ takes as input a trace~$\sigma$ and a prefix of length~$l$, and returns the first~$l$ events of the trace. The prefixes are grouped into \textit{buckets} based on their similarities (such as length, process states, or events) using a \textit{bucketing mechanism}. The prefixes in each bucket are encoded as feature vectors following an \textit{encoding mechanism}. The buckets of feature vectors are then used to train a predictive model underpinned by a (machine) \textit{learning algorithm}. Since the future state for each case is known from the training data, pairs of the encoded prefix and the future state are used to train a predictive model for each bucket. %During the online phase, the future state for a running trace is predicted by identifying the appropriate bucket, using an appropriate encoding, and finally applying the above trained predictive model. 

%The predictive process monitoring approach used for predicting the future state of a case, such as the outcome label or remaining time for case completion, consists of two phases~\cite{teinemaa2019,verenich2019}. %a review of related studies consists of two phases. 
%The first is an \textit{offline} training phase where a predictive model (which is often a machine learning model) is trained using event log data of historical process executions; and the second is an \emph{online} stage where the future state of a running case is predicted using the trained model from the offline phase (see Fig.~\ref{fig:prediction_workflow}). 

%Finally, the classifier for the relevant bucket is used to predict the outcome label or remaining time, given the encoded features of the trace. 

%\paragraph{Bucketing, Encoding, and Learning Algorithms.}

%\paragraph{Evaluation Measures.}

%Existing predictive process monitoring methods are built on different combinations of bucketing mechanisms, encoding mechanisms, and learning algorithms. The two predictive process monitoring benchmarks~\cite{teinemaa2019,verenich2019} evaluate these methods using the following quality measures: 
%\begin{itemize}
%	\item \textit{Accuracy}: for outcome-oriented prediction, this is measured by the \textit{area under the ROC curve} (AUC) metric; and for remaining time prediction, this is measured by the \textit{mean absolute error} (MAE) metric. Higher the AUC, better the model is at predicting and distinguishing the outcomes. MAE for remaining time prediction is the absolute difference between the actual remaining time and predicted remaining time and a lower MAE indicates better performance of the predictive model.
%	\item \textit{Earliness}: in both predictions, this is defined as the smallest prefix length with the desired level of accuracy. 
%\end{itemize}
%AUC indicates how well a predictive model is capable of of distinguishing between classes.
%To gain deeper insights, we analyze the interpretability of these benchmarks as discussed in Sect.~\ref{sec:reviewbenchmarks}.

